Measurement of the exclusive $\gamma \gamma \rightarrow \mu^+ \mu^-$ process in proton--proton collisions at $\sqrt{s}=13$ TeV with the ATLAS detector

The production of exclusive $\gamma \gamma \rightarrow \mu^+ \mu^-$ events in proton--proton collisions at a centre-of-mass energy of 13 TeV is measured with the ATLAS detector at the LHC, using data corresponding to an integrated luminosity of 3.2 fb$^{-1}$. The measurement is performed for a dimuon invariant mass of 12 GeV $<m_{\mu^+\mu^-}<$ 70 GeV. The integrated cross-section is determined within a fiducial acceptance region of the ATLAS detector and differential cross-sections are measured as a function of the dimuon invariant mass. The results are compared to theoretical predictions that include corrections for absorptive effects.

==> sections/Auxiliary.tex <==


%\subsection{Control distributions}
 %Control distributions of the single-muon and dimuon transverse momentum for events satisfying the selection criteria are shown in Figure~\ref{fig:MumuFinalKin}.
 %The MC predictions for the shapes of muon distributions are found to be in good agreement with the data.


\begin{figure}[!htbp]
\begin{center}
 \includegraphics[width=.49\textwidth]{figures/results/3PtllCut-mumuOS-ZBoson-h_ZDeltaPt.pdf}\put(-105,-8){{\footnotesize(a)}}
 \includegraphics[width=.49\textwidth]{figures/results/3AcoCut-mumuOS-ZBoson-h_ZptZoom.pdf}\put(-105,-8){{\footnotesize(b)}}
\end{center}
 \caption{Control distributions of (a) dimuon transverse momentum difference and (b) dimuon total transverse momentum for events passing selection requirements.
For (b) a cut on the dimuon acoplanarity ($<0.02$) is used, instead of the total transverse momentum requirement. Data are shown as points with statistical error bars, while the histograms represent the signal and background processes.   
The uncertainty band includes the MC statistical and systematic uncertainties.  
The exclusive and S-diss yields are determined from the fit
described in the text.}
\label{fig:MumuFinalKin}
\end{figure}


\graphicspath{{./figures/results/}}
\begin{figure}[!htbp]
\begin{center}
 \includegraphics[width=.5\textwidth]{3PtllCut-mumuOS-Muon-h_MuonPt.pdf}\put(-105,-8){{\footnotesize(a)}}
 \includegraphics[width=.5\textwidth]{3PtllCut-mumuOS-Muon-h_MuonEta.pdf}\put(-105,-8){{\footnotesize(b)}}
 
 \includegraphics[width=.5\textwidth]{3PtllCut-mumuOS-ZBoson-h_Zrapidity.pdf}\put(-105,-8){{\footnotesize(c)}} 
 \includegraphics[width=.5\textwidth]{3PtllCut-mumuOS-ZBoson-h_ZDeltaEta.pdf}\put(-105,-8){{\footnotesize(d)}}
\end{center}
 \caption{Control distributions of (a) single-muon transverse momentum, (b) single-muon pseudorapidity, (c) dimuon rapidity and (d) dimuon pseudorapidity difference. 
  Data are shown as points with statistical error bars, while the histograms represent the signal and background processes.   
The uncertainty band includes the MC statistical and systematic uncertainties.  
The exclusive and S-diss yields are determined from the fit
described in the text. }
\label{fig:MumuDeltaFinalKin}
\end{figure}




\graphicspath{{./figures/}}
\begin{figure}[!htbp]
\begin{center}
 \includegraphics[width=.5\textwidth]{fit_dphi_12.pdf}\put(-105,-8){{\footnotesize(a)}}
 \includegraphics[width=.5\textwidth]{fit_dphi_17.pdf}\put(-105,-8){{\footnotesize(b)}}
 
 \includegraphics[width=.5\textwidth]{fit_dphi_22.pdf}\put(-105,-8){{\footnotesize(c)}}
 \includegraphics[width=.5\textwidth]{fit_dphi_30.pdf}\put(-105,-8){{\footnotesize(d)}}
\end{center}
 \caption{Dimuon acoplanarity distribution after signal selection requirements for different dimuon invariant mass regions: (a) $12~\GeV{} <m_{\mu^+\mu^-}<17~\GeV{}$, (b) $17~\GeV{} <m_{\mu^+\mu^-}< 22~\GeV{}$, (c) $22~\GeV{} <m_{\mu^+\mu^-}< 30~\GeV{}$ and (d) $30~\GeV{} <m_{\mu^+\mu^-}< 70~\GeV{}$.
 Data are shown as points with
statistical error bars, while the histograms, in top-to-bottom order, represent the simulated exclusive signal, 
the S-diss and the sum of D-diss and DY backgrounds.
The exclusive and S-diss yields are determined from the fit
described in the text. The last bin in each of the distributions includes overflow events.}
\label{fig:fitMumuYieldMBins}
\end{figure}


\begin{figure}[!htbp]
\begin{center}
 \includegraphics[width=.55\textwidth]{0PreselectionPt1GeV-mumuOS-Tracking-h_Trkz0LV_3mm.pdf}
\end{center}
 \caption{Demonstration of the modelling of longitudinal impact parameter for events with one additional extra track near the dimuon vertex. The absolute difference in $z$ of the extra track and the dimuon vertex is shown in the region defined by $\pt^{\mu^+\mu^-}< 1~\GeV{}$ and $12~\GeV{} <m_{\mu^+\mu^-}< 70~\GeV{}$. One and only one extra track is required within $|z_0^{\textrm{trk}}| = 3$~mm window.}
\label{fig:Unfold1}
\end{figure}


\begin{figure}[!htbp]
\begin{center}
 \includegraphics[width=.45\textwidth]{figures/results/mass_response_mumu.pdf}\put(-105,-8){{\footnotesize(a)}}
 \vspace{-0.0005in}
 \includegraphics[width=.45\textwidth]{figures/results/mass_purity_mumu.pdf}\put(-105,-8){{\footnotesize(b)}}
\end{center}
 \caption{(a) Unfolding response matrix and (b) estimated signal purity corresponding to $m_{\mu^+\mu^-}$ as obtained with signal MC sample. The bin widths are chosen to ensure the signal purity above 90\%.}
\label{fig:Unfold2}
\end{figure}




\begin{landscape}

\begin{figure}[!htbp]
\begin{center}
 \includegraphics[width=1.2\textwidth]{vp1_final_run280673_evt272199949.png}
\end{center}
 \caption{Event display for exclusive \gmgmmumu candidate. Event 272199949 from run 280673 taken on 2015.09.29 at 15:30:59 is shown. The dimuon pair has $m_{\mu^+ \mu^-}=\SI{13.3}{\GeV}$, $p_{\mathrm{T}}^{\mu^+ \mu^-}=0.8~\GeV{}$ and acoplanarity = 0.01.
 The top right insert presents a zoom on the proton--proton interaction region in the longitudinal view, with a further zoom on the region around the dimuon vertex.}
\label{fig:EvtDispMuons}
\end{figure}

\end{landscape}





